Distinguishing Learning Rules with Brain Machine Interfaces

Despite extensive theoretical work on biologically plausible learning rules, clear evidence about whether and how such rules are implemented in the brain has been difficult to obtain. We consider biologically plausible supervised- and reinforcement-learning rules and ask whether changes in network activity during learning can be used to determine which learning rule is being used. Supervised learning requires a credit-assignment model estimating the mapping from neural activity to behavior, and, in a biological organism, this model will inevitably be an imperfect approximation of the ideal mapping, leading to a bias in the direction of the weight updates relative to the true gradient. Reinforcement learning, on the other hand, requires no credit-assignment model and tends to make weight updates following the true gradient direction. We derive a metric to distinguish between learning rules by observing changes in the network activity during learning, given that the mapping from brain to behavior is known by the experimenter. Because brain-machine interface (BMI) experiments allow for precise knowledge of this mapping, we model a cursor-control BMI task using recurrent neural networks, showing that learning rules can be distinguished in simulated experiments using only observations that a neuroscience experimenter would plausibly have access to.

==> author-checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See, the Discussion}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We emphasize important assumptions in the main text, and derive more extensive proofs in the Appendix}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{Proofs are included in the Appendix}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code included as supplementary material}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Appendix}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{All simulations were run on a CPU}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> miscellaneous.tex <==
%%%%% SECTIONS REMOVED FROM MAIN TEXT AND APPENDIX


\textbf{Covariance Metric}. We can construct a different, but related metric based on covariance of neural activity.

\begin{equation}
\Delta \mathrm{Cov}(h^t)^{\mathrm{data}} =     \mathrm{Cov}(h^{t,\mathrm{after}}) - \mathrm{Cov}(h^{t, \mathrm{before}}) 
\end{equation}

\begin{equation}
\Delta \mathrm{Cov}(h^t)^{\mathrm{pred}} =     \mathrm{Cov}(h^{t,\mathrm{before}} + \Delta h) - \mathrm{Cov}(h^{t,\mathrm{before}}) 
\end{equation}

\begin{equation}
\Delta \mathrm{Cov}(h^t)^{\mathrm{pred}} =     \mathrm{Cov}(h^{t,\mathrm{before}} + \Delta \mathbf{W}^{\mathrm{rec}} h^{t-1,\mathrm{before}}) - \mathrm{Cov}(h^{t,\mathrm{before}}) 
\end{equation}


% $$\mathbf{F}^{\text{late}}(\mathbf{h}^*)$$




% $$\Delta\mathbf{F}^{\text{data}}(\mathbf{h}^*) \approx \Delta \mathbf{W}^{\text{rec}} \mathbf{h}^*$$

% for any given vector of neural activity $\mathbf{h}^*$. 

% We can then calculate a gradient correlation index for the two predictions. For the supervised learning rule that depends explicitly on $\mathbf{M}$:

% $$\text{GCI}(\mathbf{M}) = \sum_{\mathbf{h}} \frac{\Delta\mathbf{F}^{\text{pred}}(\mathbf{h} | \mathbf{M}) \cdot \Delta\mathbf{F}^{\text{data}}(\mathbf{h})}{|\Delta\mathbf{F}^{\text{pred}}(\mathbf{h} | \mathbf{M}) ||\Delta\mathbf{F}^{\text{data}}(\mathbf{h})|}$$



% and for the model-free reinforcement learning case, which implicitly aligns with the true readout $\mathbf{W}^{\text{bmi}}$:

% $$\text{GCI}(\mathbf{W}^{\text{bmi}}) = \sum_{\mathbf{h}} \frac{\Delta\mathbf{F}^{\text{pred}}(\mathbf{h} | \mathbf{W}^{\text{bmi}}) \cdot \Delta\mathbf{F}^{\text{data}}(\mathbf{h})}{|\Delta\mathbf{F}^{\text{pred}}(\mathbf{h} | \mathbf{W}^{\text{bmi}}) ||\Delta\mathbf{F}^{\text{data}}(\mathbf{h})|}$$

% A higher $\text{GCI}(\mathbf{M})$ indicates that the data is more strongly correlated with a learning rule that is biased by some internal model of credit assignment $\mathbf{M}$.


% There are a few other possible ways to do something in this vein. We could, for example, look at the change in the covariance matrices before, during and after learning, and compare the data with our prediction.

% \begin{equation*}
%     \Delta \mathbf{C}^{\mathrm{data}} = \mathbf{C}_{\mathrm{after}}^{\mathrm{data}} - \mathbf{C}_{\mathrm{before}}^{\mathrm{data}} 
% \end{equation*}
% where we define the data covariance matrix $\mathbf{C}_{\mathrm{after}}^{\mathrm{data}} = \frac{1}{T} \mathbf{H}_{\mathrm{after}} \mathbf{H}_{\mathrm{after}}^\top$. We could then compare the \textit{predicted} change in covariance matrices in a similar manner to equation (\ref{correlation}) above.

% %%%%%%%%%%%%%%%%
% %   FIGURE 3   %
% %%%%%%%%%%%%%%%%
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/fig3-2022-5-5.png}
%   \caption{Further scenarios. (A) RNNs where internal model $\mathbf{M}$ is improving, i.e. increasingly aligning with the true readout $\mathbf{W}^{\mathrm{rec}}$. Early on in learning, the change in activity is distinguishable via our flow field metric, while late in training there is less bias in learning. (B) RNNs where the only learned weights are $\mathbf{W}^{\mathrm{fb}}$, after pretraining $\mathbf{W}^{\mathrm{rec}}$. The learning rule for feedback weights uses a fixed $\mathbf{M}$. After learning, the feedback weights themselves are more aligned with $\mathbf{M}$ weights than $\mathbf{W}^{\mathrm{bmi1}}$. (C) For same hyperparameters as in Figure 2, it is much harder to determine bias. (D) RNNs where feedback weights are learned with biased RFLO, and recurrent weights are learned with REINFORCE. (E) Learning with two sets of weights leads to faster task improvement. (F)  }
% \end{figure}




%\section{Neural signatures of learning with and without model of credit assignment are distinct}










% Put this in the appendix
%Looking at neural activity at a subsequent trial, and linearizing about a fixed point:

% $$h_i^t + \Delta h_i^t \approx (1-\frac{1}{\tau})h_i^{t-1} + \frac{1}{\tau} \phi(\sum_j W_{ij}^{\text{rec}}h_j^{t-1}) + \frac{1}{\tau} \phi'(\sum_j W^{\text{rec}}_{ij} h_j^{t-1}) \sum_k \Delta W^{\text{rec}}_{ik} h_k^{t-1}$$

%so we can therefore treat the \textit{change in neural activity} between trials at time step $t$ as the following expression:

% $$\Delta h_i^t = \frac{1}{\tau} \phi'(\sum_j W^{\text{rec}}_{ij} h_j^{t-1}) \sum_k \Delta W^{\text{rec}}_{ik} h_k^{t-1}$$
%If we approximate $\phi(x) = x$, then we arrive at a linear approximation to the change in neural activity between trials:

% \begin{equation}
% \label{activity_h_propto}
%   \Delta h_i^t \propto \frac{1}{\tau} \sum_k \Delta W^{\mathrm{rec}}_{ik} h_k^{t-1} 
% \end{equation}

% If the learning rule is linear, then the weights will always update along the same high-dimensional plane. This allows us to get a linear expression for the total change in neural activity over many trials.

% \begin{equation}
%    \sum_{\mathrmm{trials}} \Delta h_i^t \propto \frac{1}{\tau} \sum_{\mathrmm{trials}} \sum_k \Delta W^{\mathrm{rec}}_{ik} h_k^{t-1} 
% \end{equation}












% \subsection{Neural activity updated via reinforcement learning is proportional to ``true'' $\mathbf{W}^\mathrm{bmi}$ readout with isotropic Gaussian noise}

% NOTE - INDICES NEED TO BE CLEANED UP HERE

% We can do the same exercise for the RL scenario, and show that the change in neural activity due to an RL update will follow the ``true'' gradient proportional to $\mathbf{W}^{\text{bmi}}$

% For RL, we define a scalar reward as $R^t = -\frac{1}{2}|\epsilon(t)|^2$, either defined at each timestep or at the end of each trial

% At each time step during a trial, noise is added to each hidden/recurrent unit such that $h_i^t \rightarrow h_i^t + \xi_i$, where $\xi \sim \mathcal{N}(0,\sigma^2)$

% We've defined our RL update rule as

% $$\Delta W_{ij}^{\text{rec}} = \eta (R^t - \bar{R}^t) \overline{ \xi_i \phi'(u_i)h_j(t)}$$

% we can make the following approximation

% $$R^t - \bar{R}^t = -\frac{1}{2} |\epsilon^t|^2 - \langle R^t \rangle_{\xi} \approx -\frac{1}{2}| y^{t} -W^{\text{bmi}}_{ij} (h_j^t + \xi_j)|^2 - \langle R^t \rangle_{\xi}$$

% If we assume the noise is small, this can be expressed as (is this expansion ok?)

% $$\approx -\frac{1}{2}| \langle \epsilon^t \rangle -W^{\text{bmi}}_{ij} \xi_j|^2 - \langle R^t \rangle_{\xi}$$

% $$\approx -\frac{1}{2}|\langle \epsilon^t \rangle |^2 - \langle \epsilon^t_i \rangle W^{\text{bmi}}_{ij} \xi_j + \mathcal{O}(\xi)^2 - \langle R^t \rangle_{\xi}$$

% $$R^t - \bar{R}^t \approx \sum_{ij} \langle \epsilon^t_i \rangle W^{\text{bmi}}_{ij} \xi_j + \mathcal{O}(\xi)^2$$

% Now we can do the same exercise and plug it back in to the estimate for change in neural activity

% $$\langle \Delta h_i^t \rangle = \frac{1}{\tau} \phi'(\sum W^{\text{rec}}_{ij} h_j^{t-1}) \sum_k \Big[ \langle \Delta W_{ik}^{\text{rec}} \rangle_{\xi} \Big] h_k^{t-1}$$

% $$\langle \Delta h_i^t \rangle = \frac{1}{\tau} \phi'(\sum W^{\text{rec}}_{ij} h_j^{t-1}) \sum_k \Big[ \langle \eta (R^t - \bar{R}^t) \overline{ \xi_i \phi'(u_i)h_j(t)} \rangle_{\xi} \Big] h_k^{t-1}$$

% why does $\xi$ disappear? Should we include a variance term $\sigma$?

% $$\langle \Delta h_i^t \rangle = \frac{1}{\tau} \phi'(\sum W^{\text{rec}}_{ij} h_j^{t-1}) \sum_k \eta \Big[ \sigma^2 \langle \epsilon^t_i \rangle W^{\text{bmi}}_{ik} \phi'(u_i)h_k(t) \Big] h_k^{t-1}$$

% $$\langle \Delta h_i^t \rangle = \frac{1}{\tau} \eta \sigma^2 [ (\mathbf{W}^{\text{bmi}})^{\top} \langle \epsilon^t \rangle ]_i\phi'(\sum W^{\text{rec}}_{ij} h_j^{t-1}) \sum_k \Big[ \phi'(u_i)h_k(t) \Big] h_k^{t-1}$$

% assume linearity again so that $\phi(x) =x$ and $\phi'(x) =1$

% $$\langle \Delta h_i^t \rangle = \frac{1}{\tau} \eta \sigma^2 [ (\mathbf{W}^{\text{bmi}})^\top \langle \epsilon^t \rangle ]_i \sum_k \overline{h_k(t)}  h_k^{t-1}$$

% so here we see that the change in neural activity is proportional to the ``true'' gradient defined by the readout $\mathbf{W}^{\text{bmi}}$ readout.







% \subsection{Neural activity updated via reinforcement learning is biased with either non-isotropic Gaussian noise or non-full rank Gaussian noise }

% We now relax the assumption that the noise injected to the system at every time step is isotropic Gaussian noise \cite{scott2021beyond}. At each time step during a trial, noise is added to each hidden/recurrent unit such that $h_i^t \rightarrow h_i^t + \xi_i$, where $\xi \sim \mathcal{N}(0,\Sigma)$, where $\Sigma$ is the covariance matrix. CLEAN UP INDICES HERE

% Starting again with our RL update rule:

% \begin{equation}
% \Delta W_{ij}^{\text{rec}} = \eta (R^t - \bar{R}^t) \overline{ \xi_i \phi'(u_i)h_j(t)}
% \end{equation}

% The average change in weights will be

% $$\langle \Delta W_{ij}^{\text{rec}} \rangle = \eta \big[ \sum_{kl} \langle \epsilon^t_k \rangle W^{\text{bmi}}_{kl} \xi_l + \mathcal{O}(\xi)^2 \big] \overline{ \xi_i \phi'(u_i)h_j(t)}$$

% $$\approx \eta \sum_{kl} \langle \epsilon^t_k \rangle W^{\text{bmi}}_{kl} \big( \xi_l \xi_i \big) \phi'(u_i)h_j(t)$$

% Making the approximation that $\phi'(u_i)=1$ as before, and defining $\xi_j \xi_i = \Sigma_{ji}$, we get

% $$\langle \Delta W_{ij}^{\text{rec}} \rangle \approx \eta \sum_{kl} \langle \epsilon^t_k \rangle W^{\text{bmi}}_{kl} \Sigma_{li} h_j(t)$$

% If the covariance matrix is not full rank, but has equal variance in the dimensions that are nonzero, then $W^{\text{bmi}}_{ij} \Sigma_{ji}$ will lead to a projection onto the nonzero noise subspace. If the covariance matrix is non-isotropic (and either full rank or non full rank), then $W^{\text{bmi}}_{ij} \Sigma_{ji}$ will bias the weight changes in a manner that depends on the eigenvalues of $\Sigma$.

% NOTE: INCLUDE SCHEMATIC FIGURE HERE








%\subsubsection{Enforcing Local Update for REINFORCE Rule (à la RFLO)}
% The term $ \frac{\partial h_j(t-1)}{\partial W_{ab}} $ includes both \textit{local} and \textit{nonlocal} terms \cite{murray2019local}. However, we can separate the local and nonlocal weights and take the derivative:
% \begin{equation}
%     = \frac{\partial}{\partial W_{ab}}\Big[  \phi \Big(\sum_j W_{ij} \cdot h_j(t-1) \Big)_{i \neq a} + \delta_{ia} \phi \Big(\sum_j W_{aj} \cdot h_j(t-1) \Big) \Big] 
% \end{equation}
% The derivative of the local term is simply:
% \begin{equation}
%     \frac{\partial}{\partial W_{ab}}\Big[ \delta_{ia} \phi \Big(\sum_j W_{ij} \cdot h_j(t-1) \Big) \Big] = \delta_{ia} \phi' \Big(\sum_j W_{ij} \cdot h_j(t-1) \Big) h_b(t-1)
% \end{equation}
% Keeping only the expression for the local terms, we arrive at:
% \begin{equation}
%     \frac{\partial}{\partial W_{ab}} \ln(\pi(z_i|t,W)) = -\frac{1}{\sigma} \xi \Bigg( (1-\frac{1}{\tau}) \frac{\partial h_i(t-1) }{\partial W_{ab}} - \frac{1}{\tau}  \delta_{ia} \phi' \Big(\sum_j W_{ij} \cdot h_j(t-1) \Big) h_b(t-1) \Bigg)
% \end{equation}
% Following RFLO, the recursive relation of the derivative with only \textit{local} terms is:
% \begin{equation}
%     \frac{\partial h_i(t-1) }{\partial W_{ab}}  = (1-\frac{1}{\tau}) \frac{\partial h_i(t-2) }{\partial W_{ab}} - \frac{1}{\tau}  \delta_{ia} \phi' \Big(\sum_j W_{ij} \cdot h_j(t-2) \Big) h_b(t-2)
% \end{equation}
% This therefore defines the eligibility trace. These two coupled, recursive equations can be expressed as:
% \begin{equation}
%     \overline{ \nabla_{W} \ln(\pi(z|t,W))}
% \end{equation}
% Finally, we can construct an update rule:
% \begin{equation}
%     \Delta W_{ij} = \eta (R^t - \bar{R}^t) \overline{ \nabla_{W} \ln(\pi(z|t,W))}
% \end{equation}
% where $(R^t - \bar{R}^t)$ is the return.
% where $R^T$ is:
% \begin{equation}
% R^t = -(\mathrm{distance \; to \; target})^2 - \lambda |\textbf{y}^t|^2
% \end{equation}
% \begin{equation}
%     W_{ij}(t+1) =  W{ij}(t) + \Delta W_{ij}
% \end{equation}


\textbf{Experimental Setup 1}: Train a nonhuman primate to proficiency with decoder $\mathbf{W}^{\mathrm{bmi}0}$, then change the decoder to $\mathbf{W}^{\mathrm{bmi}1}$, and record neural activity during learning.  If a nonhuman primate is using some kind of internal model of credit assignment $\mathbf{M}$ for learning immediately after switching decoders, we can hypothesize that matrix $\mathbf{M}$ is equivalent or similar to $\mathbf{W}^{\mathrm{bmi}0}$. Given this straightforward setup, we can ask whether the change in neural activity is better predicted by decoder $\mathbf{W}^{\mathrm{bmi}0}$ or by $\mathbf{W}^{\mathrm{bmi}1}$ using the framework outlined above.

\textbf{Experimental Setup 3}: \citet{golub2015internal} proposed an intriguing technique called Internal Model Estimation (IME) for statistically estimating a monkey's ``internal model'' for BMI control. The authors noted that even during proficient cursor control, monkeys sometimes moved the cursor in a circuitous manner or occasionally made errors, and hypothesized that these errors were likely due to a mismatch between a subject's ``internal model'' and the BMI mapping. As in setups 1 and 2, train a nonhuman primate to proficiency with decoder $\mathbf{W}^{\mathrm{bmi}0}$, then change the decoder to $\mathbf{W}^{\mathrm{bmi}1}$, and record neural activity during learning. Estimate some internal model $\hat{\mathbf{M}}$ using IME, and then ask whether the change in neural activity is better predicted by decoder $\hat{\mathbf{M}}$ or by $\mathbf{W}^{\mathrm{bmi}1}$.

We simulate this setup and show that for supervised learning with RFLO [\textbf{explain setup here}]


\textbf{Learning Recurrent and Feedback Weights Simultaneously} There is ample behavioral and physiological evidence that motor learning occurs on at least two timescales; a short timescale likely mediated by cerebellum, and a longer timescale possibly mediated by the basal ganglia \cite{athalye2020neural}. We therefore applied our analysis to networks with a supervised learning rule in upstream weights $\mathbf{W}^{\mathrm{fb}}$ and a reinforcement learning rule in recurrent weights $\mathbf{W}^{\mathrm{rec}}$.  We found that when the learning rate of $\mathbf{W}^{\mathrm{rec}}$ was much slower than the learning rate of $\mathbf{W}^{\mathrm{fb}}$, we were indeed able to see that the changes in neural activity aligned with $\mathbf{W}^{\mathrm{bmi1}}$.




%   \caption{Gradients are distinguishable between biased and unbiased learning rules (A) Experimental setup: pretrain a single network with decoder $W^{\mathrm{bmi}0}$, change decoder to $W^{\mathrm{bmi}1}$ and then train two identical networks with RFLO and REINFORCE. For RFLO, we control alignment of $\mathbf{M}$ (B) Alignment of (cumulative average) weight change $\Delta \mathbf{W}^{\mathrm{rec}}$ with decoders $\mathbf{W}^{\mathrm{bmi}0}$,$\mathbf{W}^{\mathrm{bmi}1}$ and $\mathbf{M}$ for RFLO. For RFLO, we set $\mathbf{M} \angle W^{\mathrm{bmi}1}=0.6$ (C) Alignment of  (cumulative average) weight change $\Delta \mathbf{W}^{\mathrm{rec}}$ with decoders for REINFORCE (D) Correlation of predicted vs. measured change in covariance for RFLO (E) Correlation of predicted vs. measured change in covariance for REINFORCE (F) RFLO flowfield alignment across choices of M (G) REINFORCE flow field alignment across choices of $\mathbf{W}^{\mathrm{bmi}0}$}





%of the form:
%\begin{equation}\label{weight_update}
%\Delta W_{ij}^{\mathrm{rec}} = \frac{\partial L}{\partial W_{ij}^{\mathrm{rec}}} \propto \boldsymbol \eta \Big[ (\mathbf{W}^{\mathrm{bmi}} )^\top \epsilon^t\Big]_i \frac{\partial h^t_i}{\partial W_{aj}^{\mathrm{rec}}}
%\end{equation}
%\begin{equation}
%    \label{eqn-rflo-dhdW}
%    \frac{\partial h^t_i}{\partial W_{aj}^{\mathrm{rec}}} \approx \big( 1- \frac{1}{\tau}\big) \frac{\partial h^{t-1}_i}{\partial W_{aj}^{\mathrm{rec}}} + \frac{1}{\tau}\delta_{ia} \phi'(u_a^t)h_j^{t-1} + \hcancel{ \frac{1}{\tau} \phi'(u_k^t) W_{kl} \frac{\partial h_l^{t-1}}{\partial W^{\mathrm{rec}}_{aj}}} 
%\end{equation}
%where the final term in equation (\ref{eqn-rflo-dhdW}) is discarded.


%Note in particular the appearance of $\mathbf{W}^\mathrm{bmi}$ in \ref{eq:weight_update}, which assigns credit for the readout error to each postsynaptic unit $i$.  
%that, for a given presynaptic unit $j$, the updates are proportional to the transpose of the BMI readout set by the experimenter, $\mathbf{W}^\mathrm{bmi}$.
% Experiments of this kind typically train the monkey to control a cursor given one decoder, and then \textit{change} the decoder (either slightly or drastically) \cite{sadtler2014neural,golub2018learning,oby2019new}. The monkey then has to learn to control the cursor well again. When the experimenter changes the decoder to weights $\mathbf{W}^\mathrm{bmi}$, the chances that the monkey somehow has a perfect estimate of the \textit{transpose} of $\mathbf{W}^\mathrm{bmi}$ as in equation (\ref{eq:weight_update}) are very low, i.e. even after learning, the estimate is likely to remain imperfect \cite{golub2015internal}. If this matrix is completely random, the network won't learn at all, since the feed forward decoder $\mathbf{W}^\mathrm{bmi}$ is fixed. However, if there is a \textit{separate} feedback matrix $\mathbf{M}$ that is \textit{partially} aligned with the decoder $\mathbf{W}^\mathrm{bmi}$, then learning \textit{can} occur. We can define some matrix $\mathbf{M}$, and conceptually think about this matrix as the monkey's \textbf{biased, internal model of credit assignment}. With this in mind, a more likely learning rule would have this form:
% \begin{equation}\label{eq:weight_update_M}
% \Delta W_{ij}^\mathrm{rec} = 
%     \eta \sum_{t=1}^T 
%     \left[\mathbf{M} \boldsymbol{\epsilon}^t\right]_i
%     p_{ij}^t
% \end{equation}
% Our learning rule therefore makes two key approximations: (i) it avoids the weight transport problem by replacing $(\mathbf{W}^\mathrm{bmi})^\top$ with $\mathbf{M}$, and (ii) it avoids issues of locality by approximating $\partial h^t_i / \partial W_{aj}^{\mathrm{rec}}$. Whereas RFLO as it appears in \citet{murray2019local} randomly selects for matrix $\mathbf{M}$ and allows learning in $\mathbf{W}^\mathrm{bmi}$, here we choose and fix $\mathbf{W}^\mathrm{bmi}$, and do not allow any learning.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Changes in weights lead to changes in activity %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textbf{Changes in weights lead to changes in activity.} Experimentally, it is typically not possible to detect changes in the synaptic weights themselves at the scale of large neural populations. However, experiments \textit{do} have access to the neural activity $\mathbf{h}^t$. With some approximations, we argue that the change in neural activity during learning (for a single trial and over trials) $\Delta \mathbf{h}$ is in the image of the matrix defined by the change in weights $\Delta \mathbf{W}^{\mathrm{rec}}$. 


% For the SL rule, we see that the change in neural activity during learning is directly proportional to the biased model of credit assignment $\mathbf{M}$.
% \begin{equation}
%     \Delta h_i^t \bigg|_{SL} \approx \frac{1}{\tau} \sum_k \Delta W^{\mathrm{rec}}_{ik} \bigg|_{SL} h_k^{t-1} = \frac{1}{\tau} \eta \sum_k \bigg[ \big[ \mathbf{M} \boldsymbol \epsilon^t \big]_i   \overline{h_k^t} \bigg] h_k^{t-1}
% \end{equation}
% where $\overline{h_k^t}$ is the eligibility trace defined in equation (\ref{eq:eligibility-trace}). For the RL rule, we show in Appendix \ref{sec:expected-learning-rules} that the average change in neural activity implicitly (and noisily) follows the gradient of the loss defined by the true decoder readout $\mathbf{W}^{\mathrm{bmi}}$:
% \begin{equation}\label{eq:reinforce-Wtrue}
%     \langle \Delta h_i^t \rangle \bigg|_\mathrm{RL} \approx \frac{1}{\tau} \sum_k \Delta W^{\mathrm{rec}}_{ik} \bigg|_{RL} h_k^{t-1} = \frac{1}{\tau} \eta  \sum_k \bigg[ \sigma^2 [ (\mathbf{W}^{\mathrm{bmi}})^\top \langle \epsilon^t \rangle ]_i  \overline{h_k^t} \bigg] h_k^{t-1}
% \end{equation}
% In this case, we see that the change in neural activity is proportional to the (transpose of the) BMI readout matrix itself. The question then becomes: can we practically distinguish between learning rule (\ref{eq:weight_update}) and ``biased'' learning rule (\ref{eq:weight_update_M}) using ``observable'' neural data acquired during the course of leaning? We now show how this framework can be used to detect bias in the learning update.


% The simplest form of this node perturbation algorithm would look like:
% \begin{equation}
%     \Delta W_{ij}^{\mathrm{rec}} = \eta \sum_t^T (R^t - \bar{R}^t) \xi_i^t h_j^{t-1}
% \end{equation}
% for $t = \{1,...,T\}$ where $\bar{R}^t$ is the expected reward and the term $(R^t - \bar{R}^t)$ is the reward prediction error (RPE). A more elaborate version incorporates the eligibility trace from equation (\ref{eq:eligibility-trace}) above (see Appendix \ref{sec:reinforce-derivation} for a principled derivation):
% \begin{equation}
%     \label{eq:reinforce}
%     \Delta W_{ij}^{\mathrm{rec}} = \eta \sum_t^T (R^t - \bar{R}^t) \xi_i^t p_{ij}^t 
% \end{equation}
% where $p_{ij}^t \approx \partial h_i^t /\partial W_{ij}^\mathrm{rec}$, as in equation \ref{eq:eligibility-trace}.





%\textbf{Metric for Distinguishing Bias in Neural Activity with Vector Flow Fields.} 
%We assume that we have the following (hypothetical) experimental setup. A monkey is trained to proficiently perform a BMI center-out reach task with $\mathbf{W}^{\mathrm{bmi}0}$. The experimenter then changes the decoder $\mathbf{W}^{\mathrm{bmi}0} \rightarrow \mathbf{W}^{\mathrm{bmi}1}$, and the monkey learns to perform the task well over many trials. How can we say something about the bias in learning mechanism? 

%One possible approach is to calculate the alignment/correlation between the data recorded during learning and the change in activity predicted by the decoder $\mathbf{W}^{\mathrm{bmi}1}$.


% There are many proposed algorithms for learning in artificial neural networks. Can we say something about what kind of learning mechanism is being used in a ``real'' neural circuit? Brain Machine Interface (BMI) experiments in monkeys provide interesting constraints on this particular question. We argue that BMI experiments could potentially be designed to distinguish between different learning mechanisms.

%Recent work, however, has argued that effective supervised learning in both feedforward networks and RNNs can still take place as long as there is a positive overlap between the true readout weights and the credit assignment matrix used for learning \cite{lillicrap2016random,murray2019local}. 
%If an agent is to use a credit-assignment model at all in such a task, such a model must consist of a weight matrix that imperfectly approximates the readout mapping $(\mathbf{W}^\mathrm{bmi1})^\top$, i.e.~a \textit{biased} internal model of credit assignment.


%it does not yet address the question of how to determine which credit-assignment mapping should be used in order to draw this comparison.
%This alone is something that we think is worth calculating in an experimental BMI setting. 
%However our framework is meant to disambiguate between two alternative hypotheses; i.e. given two matrices $\mathbf{M}$ and some decoder $(\mathbf{W}^{\mathrm{bmi}})^\top$, which one gives a better prediction of the change in neural activity during learning?
%While $\mathbf{W}^{\mathrm{bmi1}}$ is fixed by the experimenter,
